RIS Assisted Device Activity Detection with Statistical Channel State Information

This paper studies reconfigurable intelligent surface (RIS) assisted device activity detection for grant-free (GF) uplink transmission in wireless communication networks. In particular, we consider mobile devices located in an area where the direct link to an access point (AP) is blocked. Thus, the devices try to connect to the AP via a reflected link provided by an RIS. Therefore, a RIS phase-shift design is desired that covers the entire blocked area with a wide reflection beam because the exact locations and times of activity of the devices are unknown in GF transmission. In order to study the impact of the phase-shift design on the device activity detection, we derive a generalized likelihood ratio test (GLRT) based detector and present an analytical expression for the probability of detection. Assuming knowledge of statistical CSI, we formulate an optimization problem for the phase-shift design for maximization of the guaranteed probability of detection for all locations within a given coverage area. To tackle the non-convexity of the problem, we propose two different approximations of the objective function. The first approximation leads to a design that aims to reduce the variations of the end-to-end channel while taking system parameters such as transmit power, noise power, and probability of false alarm into account. The second approximation can be adopted for versatile RIS deployments because it only depends on the line-of-sight component of the end-to-end channel and is not affected by system parameters. For comparison, we also consider a phase-shift design maximizing the average channel gain and a baseline analytical phase-shift design for large blocked areas. Our performance evaluation shows that the proposed approximations result in phase-shift designs that guarantee high probability of detection across the coverage area and outperform the baseline designs.

==> definitions_descriptions.tex <==
% !TEX root = research_diary.tex

\longnewglossaryentry{digital-beamforming}
{name={Digital Beamforming}, text={digital beamforming}, see={beamforming}}
{%
  Beamforming processing happends before the digital-analog converters, i.e., phases and magnitudes of the signal can be changed \cite[page 228]{dahlman20185gnrnext}.
}

\longnewglossaryentry{analog-beamforming}
{name={Analog Beamforming}, text={analog beamforming}, see={beamforming}}
{%
  Beamforming processing happends after the digital-analog converters, i.e., only phases of the signal can be changed \cite[page 229]{dahlman20185gnrnext}.
}

\longnewglossaryentry{fading}
{name={Fading}, text={fading}}
{%
  Destructive interference of multiple copies of the transmit signal \cite{dewiki:210327316}.
}

\longnewglossaryentry{diversity}
{name={Diversity}, text={diversity}}
{%
  The same information reaches the receiver on statistically independent channels \cite[Chapter 13.1.1]{molisch2005wirelesscommunications}.
}

\longnewglossaryentry{spatial-diversity}
{name={Spatial Siversity}, text={spatial diversity}, see={diversity}}
{%
  In a \gls{mimo} system, transmitting the same content over statistically independent fading channels as observed in rich scattering environments. The resulting diversity gain increases the reliability of the transmission \cite{dewiki:210327316}.
}

\longnewglossaryentry{spatial-multiplexing}
{name={Spatial Multiplexing}, text={spatial multiplexing}}
{%
  Transmitting the different information over statistically independent fading channels in MIMO systems.
}

\longnewglossaryentry{beamforming}
{name={Beamforming}, text={beamforming}}
{%
  Steer the main lobe of the antenna pattern to a specific direction. Increases the reliability, but not the average channel capacity \cite{dewiki:210327316}.
}

\longnewglossaryentry{smart-antenna}
{name={Smart Antenna}, text={smart antenna}}
{%
  Multi-element antennas with signal processing that creates or combines a certain signal \cite[Chapter 1.3.2]{bjoernson2017massivemimonetworks}.
}

\longnewglossaryentry{array-gain}
{name={Array Gain}, text={array gain}}
{%
  Linear scaling of the received \gls{snr} with the number of antennas \cite[page 185]{bjoernson2017massivemimonetworks}.
}

\longnewglossaryentry{frobenius-norm}
{name={Frobenius Norm}, text={frobenius norm}}
{%
  Matrix norm corresponding to the Euclidean norm for vector. It is the square root of the sum of the squared magnitudes of the matrix elements \cite{dewiki:205157456}.
}


\longnewglossaryentry{log-likelihood-ratio}
{name={Log-Likelihood Ratio}, text={log-likelihood ratio}, see={soft-decision}}
{%
  Technically, the logarithm of the ratio of two probabilities or likelihoods. Often used in soft-decision symbol detection, where each decoded bit is given a specific reliability. The sign of the received bit gives the detected bit value and the \gls{llr} gives the reliability of that bit value. A \gls{llr} of zero means equal probability for the bit value \cite{lntwww2019soft–insoft–outdecoder}.
}

\longnewglossaryentry{soft-decision}
{name={Soft Decision}, text={soft decision}, see={hard-decision}}
{%
  In contrast to hard decision, the actual value of the received bit is considered, only its sign \cite{lntwww2019soft–insoft–outdecoder}.
}

\longnewglossaryentry{hard-decision}
{name={Hard Decision}, text={hard decision}, see={soft-decision}}
{%
  In contrast to soft decision, only the sign of the received bit is considered, not its actual value \cite{lntwww2019soft–insoft–outdecoder}.
}

\longnewglossaryentry{moment-matching-method}
{name={Moment-Matching Method}, text={moment-matching method}}
{%
  Approximate the probability distribution of a random variable by obtaining its first and second order moments, i.e., its mean and variance. These moments are used to match/fit the parameters (shape and scale) of a Gamma distribution. This approach is done in \cite[Theorem 1]{chien2021outageprobabilityanalysis}.
}


==> glossary.tex <==
\newacronym{irs}{IRS}{intelligent reflecting surface}
\newacronym{bbu}{BBU}{base band unit}
\newacronym[firstplural=remote radio heads]{rrh}{RRH}{remote radio head}
\newacronym{psd}{PSD}{power spectral density}
\newacronym{los}{LoS}{line-of-sight}
\newacronym{nlos}{NLoS}{non-line-of-sight}
\newacronym{sdp}{SDP}{semidefinite programming}
\newacronym{iid}{i.i.d.}{independent and identically distributed}
\newacronym{pdf}{PDF}{probability density function}
\newacronym{lrt}{LRT}{likelihood ratio test}
\newacronym{glrt}{GLRT}{generalized likelihood ratio test}
\newacronym{mimo}{MIMO}{multiple-input multiple-output}
\newacronym{miso}{MISO}{multiple-input single-output}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{cdf}{CDF}{cumulative distribution function}
\newacronym{svd}{SVD}{singular value decomposition}
\newacronym{llr}{LLR}{log-likelihood ratio}
\newacronym{bs}{BS}{base station}
\newacronym{mle}{MLE}{maximum likelihood estimate}
\newacronym{mop}{MOP}{multiobjective optimization problem}
\newacronym[longplural=differences-of-convex,shortplural=DC]{dc}{DC}{difference-of-convex}
\newacronym{mm}{MM}{majorization-minimization}
\newacronym{sca}{SCA}{successive convex approximation}
\newacronym{ap}{AP}{access point}
\newacronym{upa}{UPA}{uniform planar array}
\newacronym{ris}{RIS}{reconfigurable intelligent surface}
\newacronym{pin}{PIN}{positive intrinsic-negative}
\newacronym{cccp}{CCCP}{concave-convex procedure}
\newacronym{csi}{CSI}{channel state information}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{amp}{AMP}{approximate message passing}
\newacronym{gamp}{GAMP}{generalized approximate message passing}
\newacronym{qos}{QoS}{quality of service}
\newacronym{cs}{CS}{compressed sensing}
\newacronym{mud}{MUD}{multi-user detection}
\newacronym{ce}{CE}{channel estimation}
\newacronym{gf}{GF}{grant-free}
\newacronym{noma}{NOMA}{non-orthogonal multiple access}
\newacronym{ml}{ML}{maximum likelihood}
\newacronym{map}{MAP}{maximum a posteriori}
\newacronym[longplural=angles of arrival]{aoa}{AoA}{angle of arrival}
\newacronym[longplural=angles of departure]{aod}{AoD}{angle of departure}
\newacronym{nr}{NR}{new radio}
\newacronym{mrc}{MRC}{maximum ratio combining}
\newacronym{mmse}{MMSE}{minimum mean squared error}
\newacronym{ls}{LS}{least squares}

